Differentially Private $\ell_1$-norm Linear Regression with Heavy-tailed Data

We study the problem of Differentially Private Stochastic Convex Optimization (DP-SCO) with heavy-tailed data. Specifically, we focus on the $\ell_1$-norm linear regression in the $\epsilon$-DP model. While most of the previous work focuses on the case where the loss function is Lipschitz, here we only need to assume the variates has bounded moments. Firstly, we study the case where the $\ell_2$ norm of data has bounded second order moment. We propose an algorithm which is based on the exponential mechanism and show that it is possible to achieve an upper bound of $\tilde{O}(\sqrt{\frac{d}{n\epsilon}})$ (with high probability). Next, we relax the assumption to bounded $\theta$-th order moment with some $\theta\in (1, 2)$ and show that it is possible to achieve an upper bound of $\tilde{O}(({\frac{d}{n\epsilon}})^\frac{\theta-1}{\theta})$. Our algorithms can also be extended to more relaxed cases where only each coordinate of the data has bounded moments, and we can get an upper bound of $\tilde{O}({\frac{d}{\sqrt{n\epsilon}}})$ and $\tilde{O}({\frac{d}{({n\epsilon})^\frac{\theta-1}{\theta}}})$ in the second and $\theta$-th moment case respectively.

==> bare_conf <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{dwork2006calibrating}
C.~Dwork, F.~McSherry, K.~Nissim, and A.~Smith, ``Calibrating noise to
  sensitivity in private data analysis,'' in \emph{Theory of cryptography
  conference}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2006, pp.
  265--284.

\bibitem{bassily2014private}
R.~Bassily, A.~Smith, and A.~Thakurta, ``Private empirical risk minimization:
  Efficient algorithms and tight error bounds,'' in \emph{Foundations of
  Computer Science (FOCS), 2014 IEEE 55th Annual Symposium on}.\hskip 1em plus
  0.5em minus 0.4em\relax IEEE, 2014, pp. 464--473.

\bibitem{wang2019differentially2}
D.~Wang and J.~Xu, ``Differentially private empirical risk minimization with
  smooth non-convex loss functions: A non-stationary view,'' in
  \emph{Proceedings of the AAAI Conference on Artificial Intelligence},
  vol.~33, no.~01, 2019, pp. 1182--1189.

\bibitem{wang2019differentially}
D.~Wang, C.~Chen, and J.~Xu, ``Differentially private empirical risk
  minimization with non-convex loss functions,'' in \emph{International
  Conference on Machine Learning}, 2019, pp. 6526--6535.

\bibitem{bassily2020}
R.~Bassily, V.~Feldman, K.~Talwar, and A.~Thakurta, ``Private stochastic convex
  optimization with optimal rates,'' in \emph{NeurIPS}, 2019.

\bibitem{bassily2020stability}
R.~Bassily, V.~Feldman, C.~Guzm{\'a}n, and K.~Talwar, ``Stability of stochastic
  gradient descent on nonsmooth convex losses,'' \emph{Advances in Neural
  Information Processing Systems}, vol.~33, 2020.

\bibitem{feldman2020private}
V.~Feldman, T.~Koren, and K.~Talwar, ``Private stochastic convex optimization:
  optimal rates in linear time,'' in \emph{Proceedings of the 52nd Annual ACM
  SIGACT Symposium on Theory of Computing}, 2020, pp. 439--449.

\bibitem{song2020characterizing}
S.~Song, O.~Thakkar, and A.~Thakurta, ``Characterizing private clipped gradient
  descent on convex generalized linear problems,'' \emph{arXiv preprint
  arXiv:2006.06783}, 2020.

\bibitem{su2021faster}
J.~Su and D.~Wang, ``Faster rates of differentially private stochastic convex
  optimization,'' \emph{arXiv preprint arXiv:2108.00331}, 2021.

\bibitem{asi2021private}
H.~Asi, J.~Duchi, A.~Fallah, O.~Javidbakht, and K.~Talwar, ``Private adaptive
  gradient methods for convex optimization,'' in \emph{International Conference
  on Machine Learning}.\hskip 1em plus 0.5em minus 0.4em\relax PMLR, 2021, pp.
  383--392.

\bibitem{bassily2021non}
R.~Bassily, C.~Guzm{\'a}n, and A.~Nandi, ``Non-euclidean differentially private
  stochastic convex optimization,'' \emph{arXiv preprint arXiv:2103.01278},
  2021.

\bibitem{kulkarni2021private}
J.~Kulkarni, Y.~T. Lee, and D.~Liu, ``Private non-smooth empirical risk
  minimization and stochastic convex optimization in subquadratic steps,''
  \emph{arXiv preprint arXiv:2103.15352}, 2021.

\bibitem{bassily2021differentially}
R.~Bassily, C.~Guzm{\'a}n, and M.~Menart, ``Differentially private stochastic
  optimization: New results in convex and non-convex settings,'' \emph{Advances
  in Neural Information Processing Systems}, vol.~34, 2021.

\bibitem{asi2021private2}
H.~Asi, V.~Feldman, T.~Koren, and K.~Talwar, ``Private stochastic convex
  optimization: Optimal rates in $\ell_1$ geometry,'' \emph{arXiv preprint
  arXiv:2103.01516}, 2021.

\bibitem{DBLP:conf/ijcai/XueYH021}
Z.~Xue, S.~Yang, M.~Huai, and D.~Wang, ``Differentially private pairwise
  learning revisited,'' in \emph{{IJCAI}}.\hskip 1em plus 0.5em minus
  0.4em\relax ijcai.org, 2021, pp. 3242--3248.

\bibitem{wang2020differentially}
D.~Wang, H.~Xiao, S.~Devadas, and J.~Xu, ``On differentially private stochastic
  convex optimization with heavy-tailed data,'' \emph{arXiv preprint
  arXiv:2010.11082}, 2020.

\bibitem{hu2021high}
L.~Hu, S.~Ni, H.~Xiao, and D.~Wang, ``High dimensional differentially private
  stochastic optimization with heavy-tailed data,'' \emph{arXiv preprint
  arXiv:2107.11136}, 2021.

\bibitem{kamath2021improved}
G.~Kamath, X.~Liu, and H.~Zhang, ``Improved rates for differentially private
  stochastic convex optimization with heavy-tailed data,'' \emph{arXiv preprint
  arXiv:2106.01336}, 2021.

\bibitem{barber2014privacy}
R.~F. Barber and J.~C. Duchi, ``Privacy and statistical risk: Formalisms and
  minimax bounds,'' \emph{arXiv preprint arXiv:1412.4451}, 2014.

\bibitem{kamath2020private}
G.~Kamath, V.~Singhal, and J.~Ullman, ``Private mean estimation of heavy-tailed
  distributions,'' \emph{arXiv preprint arXiv:2002.09464}, 2020.

\bibitem{liu2021robust}
X.~Liu, W.~Kong, S.~Kakade, and S.~Oh, ``Robust and differentially private mean
  estimation,'' \emph{arXiv preprint arXiv:2102.09159}, 2021.

\bibitem{tao2021optimal}
Y.~Tao, Y.~Wu, P.~Zhao, and D.~Wang, ``Optimal rates of (locally)
  differentially private heavy-tailed multi-armed bandits,'' \emph{arXiv
  preprint arXiv:2106.02575}, 2021.

\bibitem{nissim2007smooth}
K.~Nissim, S.~Raskhodnikova, and A.~Smith, ``Smooth sensitivity and sampling in
  private data analysis,'' in \emph{Proceedings of the thirty-ninth annual ACM
  symposium on Theory of computing}.\hskip 1em plus 0.5em minus 0.4em\relax
  ACM, 2007, pp. 75--84.

\bibitem{bun2019average}
M.~Bun and T.~Steinke, ``Average-case averages: Private algorithms for smooth
  sensitivity and mean estimation,'' \emph{arXiv preprint arXiv:1906.02830},
  2019.

\bibitem{dwork2014algorithmic}
C.~Dwork, A.~Roth \emph{et~al.}, ``The algorithmic foundations of differential
  privacy.'' \emph{Foundations and Trends in Theoretical Computer Science},
  vol.~9, no. 3-4, pp. 211--407, 2014.

\bibitem{vershynin2018high}
R.~Vershynin, \emph{High-dimensional probability: An introduction with
  applications in data science}.\hskip 1em plus 0.5em minus 0.4em\relax
  Cambridge university press, 2018, vol.~47.

\bibitem{zhang2018ell_1}
L.~Zhang and Z.-H. Zhou, ``$\ell\_1$-regression with heavy-tailed
  distributions,'' in \emph{Advances in Neural Information Processing Systems},
  2018, pp. 1076--1086.

\bibitem{chen2020generalized}
P.~Chen, X.~Jin, X.~Li, and L.~Xu, ``A generalized catoni’s m-estimator under
  finite $\alpha$-th moment assumption with $\alpha\in (1, 2)$,''
  \emph{Electronic Journal of Statistics}, vol.~15, no.~2, pp. 5523--5544,
  2021.

\end{thebibliography}

